Integration and Packaging

Vertically integrated (3D) combinations of sensors and electronics provide the ability to fabricate small, fine pitch pixels with very small total capacitance monolithically integrated with complex circuitry. The small capacitance, enabled by the fine pixel pitch and low interconnect capacitance available in 3D hybrid bonding, provides excellent signal/noise with moderate power. This combination enables fabrication of integrated sensors and electronics with both excellent position and time resolution. In this white paper a discussion will be presented on 3D integration advantages, ongoing projects and prospects in high energy physics and beyond.

==> workshopsymbols.tex <==
%%%%   Standard symbols for use in Snowmass Working Group Proceedings%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  basic formatting macros:%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%   text mode macros

\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\etc{{\it etc.}}
\def\etal{{\it et al.}}
\def\ibid{{\it ibid}.}

\def\Acknowledgements{\bigskip  \bigskip \begin{center} \begin{large}
             \bf ACKNOWLEDGEMENTS \end{large}\end{center}}


%  equation display macros

\def\beq{\begin{equation}}
\def\eeq#1{\label{#1}\end{equation}}
\def\eeqn{\end{equation}}

%%  multiple-line equations  (use \CR as the carriage return):

\newenvironment{Eqnarray}%
   {\arraycolsep 0.14em\begin{eqnarray}}{\end{eqnarray}}
\def\beqa{\begin{Eqnarray}}
\def\eeqa#1{\label{#1}\end{Eqnarray}}
\def\eeqan{\end{Eqnarray}}
\def\CR{\nonumber \\ }

%%  reference to an equation number:

\def\leqn#1{(\ref{#1})}

%%  sizing and bars

\def\st{\scriptstyle}
\def\sst{\scriptscriptstyle}

\def\overbar#1{\overline{#1}}
\let\littlebar=\bar
\let\bar=\overbar

\def\subscr#1{{\mbox{\scriptsize #1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  expectation values: 

\def\VEV#1{\left\langle{ #1} \right\rangle}
\def\bra#1{\left\langle{ #1} \right|}
\def\ket#1{\left| {#1} \right\rangle}
\def\vev#1{\langle #1 \rangle}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% relation symbols

\def\lsim{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}
\def\gsim{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}

\def\Im{{\rm Im}}
\def\Re{{\rm Re}}
\def\tr{{ \rm tr}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  caligraphic letters (for matrix elements, luminosity, etc.)

\def\D{{\cal D}}
\def\L{{\cal L}}
\def\M{{\cal M}}
\def\O{{\cal O}}
\def\W{{\cal W}}
\def\H{{\cal H}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  matrix operations and fractions:

\def\One{{\bf 1}}
\def\hc{{\mbox{\rm h.c.}}}
\def\tr{{\mbox{\rm tr}}}
\def\half{\frac{1}{2}}
\def\thalf{\frac{3}{2}}
\def\third{\frac{1}{3}}
\def\tthird{\frac{2}{3}}

\def\del{\partial}
\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\def\dslash{\not{\hbox{\kern-2pt $\del$}}}
\def\pslash{\not{\hbox{\kern-2pt $p$}}}
\def\ETmiss{\not{\hbox{\kern-4pt $E$}}_T}

\def\Dlr{\mathrel{\raise1.5ex\hbox{$\leftrightarrow$\kern-1em\lower1.5ex\hbox{$D$}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  high-energy physics terminology:

\def\Pl{{\mbox{\scriptsize Pl}}}
\def\eff{{\mbox{\scriptsize eff}}}
\def\CM{{\mbox{\scriptsize CM}}}
\def\GUT{{\mbox{\scriptsize GUT}}}
\def\BR{\mbox{\rm BR}}
\def\ee{e^+e^-}
\def\sstw{\sin^2\theta_w}
\def\cstw{\cos^2\theta_w}
\def\mz{m_Z}
\def\gz{\Gamma_Z}
\def\mw{m_W}
\def\gw{\Gamma_W}
\def\mt{m_t}
\def\gt{\Gamma_t}
\def\mh{m_H}
\def\gh{\Gamma_H}
\def\gmu{G_\mu}
\def\GF{G_F}
\def\alphas{\alpha_s}
\def\MSB{{\bar{M \kern -2pt S}}}
\def\msb{{\bar{\scriptsize M \kern -1pt S}}}
\def\lmsb{\Lambda_{\msb}}
\def\drb{{\bar{\scriptsize D \kern -1pt R}}}
\def\ELER{e^-_Le^+_R}
\def\EREL{e^-_Re^+_L}
\def\ELEL{e^-_Le^+_L}
\def\ERER{e^-_Re^+_R}
\def\eps{\epsilon}
\def\Kzero{K^0}
\def\Kzerobar{{\bar K}^0}
\def\Dzero{D^0}
\def\Dzerobar{{\bar D}^0}
\def\Bzero{B^0}
\def\Bzerobar{{\bar B}^0}


%%%%%%%%%%%%   units for math mode  %%%%%%%%%%%%%%%%%%%%%%%%%

\def\ifb{{\rm fb}^{-1}}
\def\eV{{\rm eV}}
\def\keV{{\rm keV}}
\def\MeV{{\rm MeV}}
\def\GeV{{\rm GeV}}
\def\TeV{{\rm TeV}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%  supersymmetry:

\def\ch#1{\widetilde\chi^+_{#1}}
\def\chm#1{\widetilde\chi^-_{#1}}
\def\neu#1{\widetilde\chi^0_{#1}}
\def\s#1{\widetilde{#1}}



%%%%%%%%%%  common journal names   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\aj{{Astronomical Journal}}%
\newcommand\araa{{Annual Review of Astron and Astrophys}}%
 \newcommand\apj{{Astrophysical Journal}}%
\newcommand\apjl{{Astrophysical Journal, Letters}}%
\newcommand\apjs{{ApJS}}%
% Astrophysical Journal, Supplement
\newcommand\ao{{Appl.~Opt.}}%
% Applied Optics
\newcommand\apss{{Ap\&SS}}%
% Astrophysics and Space Science
\newcommand\aap{{Astronomy and Astrophysics}}%
\newcommand\aapr{{A\&A~Rev.}}%
% Astronomy and Astrophysics Reviews
\newcommand\aaps{{A\&AS}}%
% Astronomy and Astrophysics, Supplement
\newcommand\azh{{AZh}}%
% Astronomicheskii Zhurnal
\newcommand\baas{{BAAS}}%
% Bulletin of the AAS
\newcommand\jrasc{{JRASC}}%
% Journal of the RAS of Canada
\newcommand\memras{{MmRAS}}%
% Memoirs of the RAS
\newcommand\mnras{{Monthly Notices of the Royal Astronomical Society}}%
\newcommand\pra{{Phys.~Rev.~A}}%
% Physical Review A: General Physics
\newcommand\prb{{Phys.~Rev.~B}}%
% Physical Review B: Solid State
\newcommand\prc{{Phys.~Rev.~C}}%
% Physical Review C
\newcommand\prd{{Physics~Review~D}}%
% Physical Review D
\newcommand\pre{{Phys.~Rev.~E}}%
% Physical Review E
\newcommand\prl{{Phys.~Rev.~Lett.}}%
% Physical Review Letters
\newcommand\pasp{{Publications of the ASP}}%
\newcommand\pasj{{PASJ}}%
% Publications of the ASJ
\newcommand\qjras{{QJRAS}}%
% Quarterly Journal of the RAS
\newcommand\jcap{{JCAP}}%
\newcommand\skytel{{S\&T}}%
% Sky and Telescope
\newcommand\solphys{{Sol.~Phys.}}%
% Solar Physics
\newcommand\sovast{{Soviet~Ast.}}%
% Soviet Astronomy
\newcommand\ssr{{Space~Sci.~Rev.}}%
% Space Science Reviews
\newcommand\zap{{ZAp}}%
% Zeitschrift fuer Astrophysik
\newcommand\nat{{Nature}}%
\newcommand\iaucirc{{IAU~Circ.}}%
% IAU Cirulars
\newcommand\aplett{{Astrophys.~Lett.}}%
% Astrophysics Letters
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}%
% Astrophysics Space Physics Research
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}}%
% Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{{Fund.~Cosmic~Phys.}}%
% Fundamental Cosmic Physics
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}%
% Geochimica Cosmochimica Acta
\newcommand\grl{{Geophys.~Res.~Lett.}}%
% Geophysics Research Letters
\newcommand\jcp{{J.~Chem.~Phys.}}%
% Journal of Chemical Physics
\newcommand\jgr{{J.~Geophys.~Res.}}%
% Journal of Geophysics Research
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}%
% Journal of Quantitative Spectroscopy and Radiative Transfer
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}%
% Mem. Societa Astronomica Italiana
\newcommand\nphysa{{Nucl.~Phys.~A}}%
% Nuclear Physics A
\newcommand\physrep{{Phys.~Rep.}}%
% Physics Reports
\newcommand\physscr{{Phys.~Scr}}%
% Physica Scripta
\newcommand\planss{{Planet.~Space~Sci.}}%
% Planetary Space Science
\newcommand\procspie{{Proc.~SPIE}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
